Heat conductance oscillations in two weakly connected charge Kondo circuits

We revisit a model describing Seebeck effect on a weak link between two charge Kondo circuits, which has been proposed in the [Phys. Rev. B 97, 085403 (2018)]. We calculate the thermoelectric coefficients in the perturbation theory assuming smallness of the reflection amplitudes of the quantum point contacts. We focus on the linear response equations for the heat conductance in three different scenarios as: Fermi liquid vs Fermi liquid, Fermi liquid vs non-Fermi liquid, nonFermi liquid vs non-Fermi liquid. The oscillations of the heat conductance as a function of the gate voltage of each quantum dot are analysed in both Fermi liquid and non-Fermi liquid regimes. We discuss possible experimental realizations of the model to observe the signatures of the non-Fermi liquid behaviour in the heat conductance measurements.

==> tc-pgf.def.tex <==
%% Copyright (C) 2011-2018 by Martin Scharrer <martin@scharrer-online.de>
%% ----------------------------------------------------------------------
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `maintained'.
%%
%% The Current Maintainer of this work is Martin Scharrer.
%%
%% This work consists of the files trimclip.dtx, adjustbox.ins
%% and the derived files trimclip.sty,
%% tc-dvips.def, tc-pdftex.def, tc-pgf.def and tc-xetex.def.
%% Further author information are located in the .def files.
%%
\ProvidesFile{tc-pgf.def}[2019/01/04 v2.2 trimclip fall-back clipping driver using PGF]
\RequirePackage{pgf}
\def\@cliptoboxdim#1{%
    \setbox#1\hbox{\begin{pgfpicture}%
        \pgfpathmoveto{\pgfqpoint\z@{-\dp#1}}%
        \pgfpathlineto{\pgfqpoint\z@{\ht#1}}%
        \pgfpathlineto{\pgfqpoint{\wd#1}{\ht#1}}%
        \pgfpathlineto{\pgfqpoint{\wd#1}{-\dp#1}}%
        \pgfpathclose
        \pgfusepathqclip
        \pgfset{inner sep=\z@,outer sep=\z@,minimum size=\z@}%
        \pgfnode{rectangle}{base west}{\usebox#1}{}{}%
        \pgfsetbaselinepointnow{\pgfpoint\z@\z@}%
    \end{pgfpicture}}%
}
\def\@clipcornersofbox#1#2#3#4#5{%
    \setbox#1\hbox{\begin{pgfpicture}%
        \pgfpathmoveto{\pgfpoint{\z@}{\ht#1-#2}}%
        \pgfpatharc{180}{90}{#2}%
        \pgfpathlineto{\pgfpoint{\wd#1-#3}{\ht#1}}%
        \pgfpatharc{90}{0}{#3}%
        \pgfpathlineto{\pgfpoint{\wd#1}{#5-\dp#1}}%
        \pgfpatharc{0}{-90}{#5}%
        \pgfpathlineto{\pgfpoint{#4}{-\dp#1}}%
        \pgfpatharc{270}{180}{#4}%
        \pgfpathlineto{\pgfpoint{\z@}{\ht#1-#2}}%
        \pgfpathclose
        \pgfusepathqclip
        \pgfset{inner sep=\z@,outer sep=\z@,minimum size=\z@}%
        \pgfnode{rectangle}{base west}{\usebox#1}{}{}%
        \pgfsetbaselinepointnow{\pgfpoint\z@\z@}%
    \end{pgfpicture}}%
}
\def\@rndframearoundbox#1#2#3#4#5#6{%
    \setbox#1\hbox{\begin{pgfpicture}%
        \adjsetlength\@tempdima{\fboxsep+.5\fboxrule}%
        \@marginbox#1\@tempdima\@tempdima\@tempdima\@tempdima%
        \edef\@tempa{#6}%
        \ifx\@empty\@tempa\else
            \@clipcornersofbox{#1}{#2}{#3}{#4}{#5}%
        \fi
        \pgfset{inner sep=\z@,outer sep=\z@,minimum size=\z@}%
        \pgfnode{rectangle}{base west}{\usebox#1}{}{}%
        \pgfusepath{}%
        \adjbox@rndframe@color
        \pgfpathmoveto{\pgfpoint{\z@}{\ht#1-#2}}%
        \pgfpatharc{180}{90}{#2}%
        \pgfpathlineto{\pgfpoint{\wd#1-#3}{\ht#1}}%
        \pgfpatharc{90}{0}{#3}%
        \pgfpathlineto{\pgfpoint{\wd#1}{#5-\dp#1}}%
        \pgfpatharc{0}{-90}{#5}%
        \pgfpathlineto{\pgfpoint{#4}{-\dp#1}}%
        \pgfpatharc{270}{180}{#4}%
        \pgfpathlineto{\pgfpoint{\z@}{\ht#1-#2}}%
        \pgfpathclose
        \pgfusepath{stroke}%
        \pgfsetbaselinepointnow{\pgfpoint\z@\z@}%
    \end{pgfpicture}}%
}
\endinput
%%
%% End of file `tc-pgf.def'.
